High Performance Scalable FPGA Accelerator for Deep Neural Networks

Low-precision is the first order knob for achieving higher Artificial Intelligence Operations (AI-TOPS). However the algorithmic space for sub-8-bit precision compute is diverse, with disruptive changes happening frequently, making FPGAs a natural choice for Deep Neural Network inference, In this work we present an FPGA-based accelerator for CNN inference acceleration. We use {\it INT-8-2} compute (with {\it 8 bit} activation and {2 bit} weights) which is recently showing promise in the literature, and which no known ASIC, CPU or GPU natively supports today. Using a novel Adaptive Logic Module (ALM) based design, as a departure from traditional DSP based designs, we are able to achieve high performance measurement of 5 AI-TOPS for {\it Arria10} and project a performance of 76 AI-TOPS at 0.7 TOPS/W for {\it Stratix10}. This exceeds known CPU, GPU performance and comes close to best known ASIC (TPU) numbers, while retaining the versatility of the FPGA platform for other applications.

==> Introduction.tex <==
\vspace{-0.5em}
\section{Introduction}\label{sec:Introduction}
Today's DNN's have shown to achieve high accuracy for a variety of applications in various domains such as object detection, image classification, speech recognition, etc.  To achieve high accuracy with DNN, the depth and complexity of DNN models have increased tremendously, thus making them highly resource intensive in terms of compute/bandwidth requirements and power consumption.  This has lead current research to focus on low precision data types as an alternative means of processing these DNN's efficiently to help in reducing the computational, memory, and bandwidth requirements \cite{TernaryFGQ, CourbariauxB16, HubaraCSEB16, HeZRS15, GuptaAGN15}.

%The reconfigurable hardware designed, must be efficient in mapping tens to hundreds of highly compute intensive layers present in DNN models efficiently to achieve high performance/watt.
%Therefore, an hardware architecture designed for DNN for high performance/watt must be efficiently able to re-use the computing resources across layers, flexible enough to handle low numeric arbitrary data types and minimize movement of data within each layer.
%As a result, expensive and power hungry computers are needed to efficiently process these networks, which has led researchers to seek ways to reduce the computational, memory, and bandwidth requirements [5] [6] [7] [8] [9].

Current DNN's exploit low numeric data types for both activation and weights (example, 2-bit, 1-bit).  These low numberic data types offer order of performance improvement in hardware over regular DNN's that perform GEMM operation on FP32 bit data type.  However, there is a trade off between using low precision data types and accuracy of DNN.  For an 8-bit activation and 8-bit weight (Google TPU), the model size of the DNN reduces by 4x with minimal drop in accuracy, improves performance, and power benefits \cite{google}.  Lowering the data types to sub 8-bit for both activation and weights results in significant accuracy loss in DNN, despite re-training at lower precision \cite{TernaryFGQ}.

We can relate low precision representation to adding noise to the pre-trained DNN.  To improve the accuracy and reduce the noise of the ternary network, Fine Grain Quantization (FGQ) technique was introduced in \cite{TernaryFGQ}, which partitions the learned weight into smaller sets of disjoint blocks (N) and then ternarizes them.  The trade off between accuracy and number of multiplications (and model size) is controlled by block size (N).  Thus, ternary networks with 8-bit activation, 2-bit weights (1,-1,0), and Dynamic Fixed Point support (DFP) can help in reducing cost of computation, and model size with smaller drop in accuracy, which forms the basis of this work.  
%In this work, we build upon the strategy proposed in\cite{TernaryFGQ}, to figure out the optimal block size for Resnet Topology without compromising on accuracy. 
%We interpret low-precision/sparse representation as adding noise to pre-trained DNNs. In Section 2 we provide a perturbation analysis of pre-trained DNNs to figure out sensitivity of key quantities that contributes to
%the final perturbation. Then, we introduce the notion of residual parameters which, when added to the perturbed network, reduces the noise and improves the accurac

Convolution operations contribute to 90\% of computations in DNN's, which mostly consist of Multiply and Add (MAC) operations.  Hardware architecture designed for DNN to achieve high performance/watt must efficiently re-use the computing resources across layers, be flexible enough to handle low numeric arbitrary data types, and minimize movement of data within each layer.  FPGA's have recently shown to perform well for low numeric data types because of their ability to map these computations to low level logic operations \cite{Nurvitadhi:2017, Duncan, BNN}.  For example, 8-2 ternary operations consisting of 8-bit activations and 2-bit weights (0,1,-1) can be realized using logic elements without the need for traditional multiplier, therfore helping in the efficient use of computing resources.  Hence, the MAC operation can be converted to simply accumulation operations.  The entire DNN computation can be implemented in the core logic using Adaptive logic Modules (ALM) \cite{Arria10} in FPGA without using any DSP's.  By using ALM's compared to the traditional DSP centric approach to perform computations that result in improved performance.  As a result, FPGA's provide the opportunity to map these custom data types into low level logic efficiently compared to GPU's that work well for computations that exhibit regular parallelism and fixed data type. 

DNN convolutions consist of four levels of loop unrolling across kernels and feature maps that provide us various design choices to extract parallelism.   The data can be partitioned into smaller portions that can be stored in the on-chip memory.  The architecture designed must also handle sequential and parallel computations present in layers with minimum data movement, and memory access, thereby increasing data re-use and locality.  In this paper, we propose a FPGA based accelerator for inferencing that can map these convolutions in a DNN efficiently, and re-use compute resources across layers with different sizes and dimensions.

%\begin{itemize}
\noindent $\bullet$ We propose an high performance and scalable FPGA accelerator to implement ResNet-50 Topology efficiently with a ternary network consisting of 8-bit activations and 2-bit weights using the ALM's in the FPGA.  To the best of our knowledge, this is the first work that tries to map the entire DNN computation into ALM's for a ternary ResNet network without using DSP's to achieve high performance.

\noindent $\bullet$ Core compute engine is designed using Optimum block size (N) which is estimated from the FGQ technique without compromising on accuracy for ResNet-50.  We efficiently implement low precision DFP computations in hardware.

\noindent $\bullet$ Complete end-to-end layer computation flow is designed to integrate different computing elements present in our design, and to efficiently manage different connections present in ResNet topology.

%\end{itemize}
\iffalse
Since convolution operations often constitute more than 90%
of the total CNN operations [2][3][4][6][11], an effective
acceleration scheme of convolution requires proper management of
the parallel computations and the organization of data storage and
access across multiple levels of memories, e.g. off-chip DRAM,
on-chip SRAM and local registers. Convolution is comprised of
four levels of loops sliding along both kernel and feature maps,
resulting in a large design space to explore various choices for
implementing parallelism, sequencing of computations, and
partitioning the large data set into smaller chunks to fit into on-chip
memory. 


To maximize the computing resource utilization, the
acceleration architecture should be fully reusable for layers
with diverse dimensions and sizes. To reduce the data
movements and memory accesses, it is essential to efficiently
manage the parallel and sequential computations of convolution
and increase the data locality and reuse.
Built upon the convolution acceleration strategy proposed
in [8], we maximize the resource utilization and minimize the
data communication for deep residual CNNs. The contributions
of this work include the following.
\item We generalize the modularized hardware accelerator to
efficiently implement extremely deep residual CNNs, or
ResNets [4], with 50 and 152 convolution layers.
\item Specific computing modules are designed for different
types of ResNet layers with high scalability and reusability.
3) A layer-by-layer computation flow is designed to integrate
these computing primitives and communicate the complex
connections of deep ResNet layers



compared to GPU due to ability to handle irregular parallelism  

%because of the advantage gained by mapping the ternary operation into low level logic in 


use low precision compact data types in 

Here we are mainly focused on the trade-off between low-precision representation and accuracy of deeper
networks, keeping an eye on power- performance factors. There is a clear need for reduction in precision for both
weights and activations (that are fetched from external memory or I/O devices) for more efficient implementation
of deeper networks. Such low-precision representation for activation demands for specialized low-precision
arithmetic ([29, 28, 21] and hardware design. For example, Google’s TPU ([15]) sets a trend for a low-precision
inference pipeline (8-bit activations, 8-bit weights). Moreover, significant research energy is being expended to
explore sub-8-bit domain of DNN representation ([13, 32, 21]), where the interplay among model size, compute,
power, and accuracy becomes more tricky. For 8-8 representation, despite reducing the model size by 4×, only
minimal drop in accuracy has been observed for deeper networks. However, the accuracy degrades significantly
in sub-8-bit domain where we reduce precisions for the weights and/or the activations, and we observe some
noticeable drop in accuracy for deeper networks despite rigorous (re)training at low-precision ([21]).




Across generations, GPUs offer increased
FLOP/s, by incorporating more floating-point units, on-chip
RAMs, and higher memory bandwidth. For example, the latest
Titan X Pascal offers peak 11 TFLOP/s of 32-bit floating-point
throughput, a noticeable improvement from the previous
generation Titan X Maxwell that offered 7 TFLOP/s peak
throughput. However, GPUs can face challenges from issues, such
as divergence, for computation that exhibits irregular parallelism.
Further, GPUs support only a fixed set of native data types. So,
other custom-defined data types may not be handled efficiently.
These challenges may lead to underutilization of hardware
resources and unsatisfactory achieved performance

Moreover, DNN algorithms are evolving rapidly. Recent
developments point toward next-generation DNNs that exploit
network sparsity [4,5,6] and use extremely compact data types
(e.g., 1bit, 2bit) [1,2,3,4,5]. These emerging DNNs offer orders of
magnitude algorithmic efficiency improvement over “classic”
DNNs that rely on dense GEMM on FP32 data type, but they
introduce irregular parallelism and custom data types, which are
difficult for GPUs to handle. In contrast, FPGAs are designed for
extreme customizability. FPGAs shine on irregular parallelism
and custom data types. An inflection point may be near!


With the rise of lower numeric precision networks using
both activation and weight data widths as low as 1-bit, FPGAs will
shine by demonstrating their capabilities in this domain. One of the
problems however is that few frameworks exist that allow FPGAs
to be easily benchmarked with a variety of low precision
configurations for several different networks. Further, there is
limited amounts of data available for CNN on new FPGA devices
such as Stratix 10 to help motivate future research. To address these
problems, we provide the following contributions:


This loss severely undermines the purpose of
deploying a deeper network with sub-8-bit representation. Also, for deeper networks we need significantly more
parameters in order to achieve even a small gain in accuracy. In Figure 1 we plot accuracy gain vs depth increase
for deeper ResNet models (w.r.t shallower ResNet-18) pre-trained on ImageNet. It is evident that the accuracy
almost saturates at ResNet-101, e.g., ResNet-200 is only < 0:8% more accurate despite being twice as deep. A
sub-8-bit solution, e.g., 8-4 (4 bit weights), if produces ∼ 2% drop on ResNet-101, might be equivalent to 8-8
on much shallower ResNet-50 in terms of model size and accuracy, but could be worse in power consumption.
This weakens the motivation for sub-8-bit representation of deeper networks. Ternary 8-2 networks ([18, 21]),
on the hand, can have some computational benefits, such as, only few multiplications, sparse operations, much
smaller model size etc. However, the biggest issue is the loss of accuracy for deeper networks. [21] introduced a fine-grained quantization (FGQ) method that first partitions the learned weights into disjoint blocks,
and then ternarizes them. The block size (N) controls the accuracy vs number of multiplications (and model
size). For smaller N = 4, the accuracy is ∼ 3% off from ResNet-101 (without any low-precision re-training),
eliminating 75% multiplications. However, to eliminate significantly more multiplications N should be higher,
e.g. N = 64. But this incurs significant loss in accuracy, although a major part of it had been recovered via
rigorous low-precision (re)training. The remaining gap in accuracy (∼ 4% gap for ResNet-50) might not be
acceptable for some applications, and/or the power-performance number might be close to that of 8-8 on a shallower network. Another limitation of existing sub-8-bit models is that the lost accuracy cannot be recovered
once deployed, and also these models cannot be set on a ‘power-saving’ mode (say, via less MAC) when some
further loss in accuracy is tolerable. They essentially operate on a ‘fixed-accuracy-fixed-power’ mode.
\fi

==> abstract.tex <==
\section{abstract}\label{sec:abstract}
%State of art Deep Neural Networks (DNN) require dense matrix multiplication (GEMM) that maps quite well on to GPU. 
Recent studies have explored low precision hardware for Deep Neural Networks (DNN) which reduces the cost of computation, movement of data, and storage requirements without compromising on accuracy.  FPGA's have shown to effectively map low precision custom data types with irregular parallelism compared to GPU's.  In this paper, we propose an optimized FPGA inferencing accelerator tailored to achieve high performance/watt for DNN, with 8-bit activations and ternary weights.  Our accelerator design features deep pipeline stages, high spatial parallelism, and makes maximum use of on-chip resources effectively with minimum data movement. 
 Our experimental results have shown that our proposed architecture can achieve peak performance of 5 Tops for a ResNet50 network in Arria10 FPGA. We also project 0.7 ToP/s/Watt on Stratix 10 running ResNet network with only ~3.9\% accuracy degradation compared to full precision. 

%These performance numbers show > 10x enhancement, compared to state of art FPGA implementation of DNN topology.




